How Many Impulses Redux

A central problem in orbit transfer optimization is to determine the number, time, direction and magnitude of velocity impulses that minimize the total impulse. This problem was posed in 1967 by T. N. Edelbaum, and while notable advances have been made, a rigorous means to answer Edelbaum's question for multiple-revolution maneuvers has remained elusive for over five decades. We revisit Edelbaum's question by taking a bottom-up approach to generate a minimum-fuel switching surface. Sweeping through time profiles of the minimum-fuel switching function for increasing admissible thrust magnitude, and in the high-thrust limit, we find that the continuous thrust switching surface reveals the $N$-impulse solution. It is also shown that a \textit{fundamental} minimum-thrust solution plays a pivotal role in our process to determine the optimal minimum-fuel maneuver for all thrust levels. We find the answer to Edelbaum's question is not generally unique, but is frequently a set of equal-$\Delta v$ extremals. We further find, when Edelbaum's question is refined to seek the number of finite duration thrust arcs for a specific rocket engine, that a unique extremal is usually found. Numerical results demonstrate the ideas and their utility for several interplanetary and Earth-bound optimal transfers that consist of up to eleven impulses or, for finite thrust, short thrust arcs. Another significant contribution of the paper can be viewed as a unification in astrodynamics where the connection between impulsive and continuous-thrust trajectories are demonstrated through the notion of \textit{optimal switching surfaces}

==> Reachability.tex <==
\section{Remarks On Reachability Analysis}\label{sec:reachability} 
One of the fundamental challenges in astrodynamics is to determine the time-specific reachability of an object (e.g., planet, asteroid, spacecraft or debris) given the time of flight and specifications of the propulsion system. In almost all of the space targeting and space situational awareness problems, information regarding the reachability of an object is deemed invaluable since such information can be used to rule out unreachable targets immediately during the optimization process or for other purposes. 
%This fact turns out to be quite an enabler since one does not have to solve and optimal control problem to figure this out. Put it another way, once an object is not reachable, it does not make sense to dedicate computational resources to solving an \textit{infeasible} problem! 

One key point in the above developments is that the optimal switch surface is just the ``top layer'' of an extremal field map with a wealth of additional information. Each profile on the surface corresponds to a particular minimum-fuel optimal transfer trajectory (states, co-states, and optimal thrust direction). These layers of extremal solution information can be plotted/stored/interpolated/analyzed for an infinity of uses, e.g., reachability analysis purposes.

In all of the considered cases, inspection of the switching surfaces shows that impulsive solutions set the lower theoretical limits on both time of flight, $(t_f-t_0)$ and minimum-$\Delta v$ (if $t_0$ and $t_f$ are specified). The latter is related to the propellant ratio through Tsiolkovsky rocket equation, $m_f/m_0 = e^{(-\Delta v/c)}$. In other words, the theoretical shortest time of flight is the time difference between the last impulse and the first impulse. On the other hand, these two time instants belong to the late-departure and early-arrival boundaries we have found for the cases that these two impulses are not applied at the initial and final times, and when $T \rightarrow \infty$. The fact that these late-departure and early-arrival boundaries are an attribute of the switching surface is obviously important. 

For sufficiently short specified time of flight and high thrust, we can expect the optimal $N^*_{\text{rev}}$ will be found to be 0 (a fraction of the first orbit). For all finite thrust cases, sweeping through $N_{\text{rev}}$ will lead to switching surfaces, which are analogous to Figures \ref{fig:ETo1989MLSS} and \ref{fig:EV_SS_Full}. For each rev, the shape of these early arrival or late departure boundaries can be expressed as a function of the sweep parameter (thrust in this case) as $t_{\text{EA}} = t_{\text{EA}}(T)$ and $t_{\text{LD}} = t_{\text{LD}}(T)$, where $t_{\text{EA}}$ and $t_{LD}$ denote the early-arrival time and late-departure time, respectively. The shortest time associated with a minimum-fuel finite-thrust trajectory can be evaluated as $t_{\text{EA}}-t_{\text{LD}}$. Moreover, it is possible to use the final mass and define a parameter to represent the mass ratio on the early-arrival boundary as
\begin{equation}
\Gamma = \frac{m_{\text{EA}}}{m_0},
\end{equation}
where $m_{\text{EA}}$ is the final mass of the spacecraft (on the early-arrival boundary). 

The knowledge of optimal thrust magnitude during minimum-time solutions is obviously very useful information. It is known that for minimum-time trajectories, thrust is always ``On'', which translates directly into the required mass through the constant mass flow rate relation $m_f = m_0 - \frac{T}{c} (t_f-t_0)$. This minimum-fuel reachability information can be used to rule out any target simply due to the lack of sufficient propellant. However, for higher thrust magnitudes, $\Gamma$ has utility for reachability analysis. Recognition of the existence of local extrema (see Section \ref{sec:choiceofset} ) proves to be crucial since the information on the  minimum-fuel switching surface that corresponds to $N_{\text{rev}}^*$  is needed for any analysis. Thus we specify the number ($N_{\text{rev}}$) of en route revolutions and solve the minimum-fuel problem for each and determine the minimum of the minima. Having this pivotal extremal, we can then construct the switching surface over the thrust range of interest and have visibility of all neighboring extremals when engaged in mission design analysis reachability. The other switching surfaces are associated with sub-optimal local extremal solutions and will definitely require more fuel and can usually be ignored. 

In some settings, one or more of these local optimal trajectories may be considered if other, secondary optimality or feasibility constraints (not specifically included in trajectory optimization) are invoked. For example, if the global extremal that resulted from the above logic passed too close to the Earth, or (heavens!) penetrated the Earth or Sun en route to the target orbit, then obviously such an un-specified constraint (in the original optimal control problem formulation) would be obvious and a ``sanity check'' filtering can be invoked to rule out such physically inadmissible solutions.  Such spurious solutions are regrettably encountered occasionally when optimal control theory is applied, because in our quest for simplicity of the formulation, not all conceivable physical inequality constraints are considered, until we see that a ridiculous extremal results. Sometimes such spurious solution indicates a need to re-formulate the optimal control problem, other times, we can see why the inadmissible extremal simply be deleted in favor of the second best local extremal that satisfies all constraints. 

A key point, however, if we have enough propulsion, a 2-impulse maneuver could get there in near zero time. On the other hand, if the max velocity is bounded by the escape speed, then, an $N_{\text{rev}} = 0$ 2-impulse Lambert solution would be the practical min-time maneuver. So , reachability is a function of $t_0$, $t_f-t_0$, maximum thrust, $T$, and phasing.  Optimal $N_{\text{rev}}$ likely depends on most of these as well...all of which can be explored one or two parameters at a time. We are providing an approach for such explorations of extremal solutions.

